A Search Engine for Discovery of Scientific Challenges and Directions

Keeping track of scientific challenges, advances and emerging directions is a fundamental part of research. However, researchers face a flood of papers that hinders discovery of important knowledge. In biomedicine, this directly impacts human lives. To address this problem, we present a novel task of extraction and search of scientific challenges and directions, to facilitate rapid knowledge discovery. We construct and release an expert-annotated corpus of texts sampled from full-length papers, labeled with novel semantic categories that generalize across many types of challenges and directions. We focus on a large corpus of interdisciplinary work relating to the COVID-19 pandemic, ranging from biomedicine to areas such as AI and economics. We apply a model trained on our data to identify challenges and directions across the corpus and build a dedicated search engine. In experiments with 19 researchers and clinicians using our system, we outperform a popular scientific search engine in assisting knowledge discovery. Finally, we show that models trained on our resource generalize to the wider biomedical domain and to AI papers, highlighting its broad utility. We make our data, model and search engine publicly available. https://challenges.apps.allenai.org/

==> tex files/context_model.tex <==

% Furthermore, an oracle router model that selects for each candidate sentence $\mathcal{X}$ the best variant based on knowledge of ground truth labels, obtains F1 scores of 0.907 and 0.896 for challenges/directions -- much higher than 

To approximate the oracle we run a host of experiments to find the best way to combine information from the learners: (i) apply average or a median on the logits, (ii) majority voting, (iii) log-odds extremization, (iv) training a router model based on the logit differences, (v) running a logistical regression with the embedding of the variations and their logits as features. The logistical regression worked best for challenges (f1 of 0.784) and simple-averaging best for directions (f1 of 0.773). All of the above results reflect an average over 5 seeds for robustness. 

To obtain an insight on the variations themselves we explore the average weights the logistical regression attributed to their features across all runs. For challenges 0.14, 0.21, 0.21, and 0.35 weights for v1,v2,v3,v4, respectively; and for directions 0.32, 0.2, 0.07 and 0.45. Interestingly this suggests that training the model end-to-end with context is preferable even when the context is not available at inference, a modelling conclusion that can potentially serve future designs in text classification problems.

To assess that the results are attributed to the described factors, and not simply to potential noise reduction that could have been achieved by sheer addition of classifiers, we compare our described technique to applying the same methods to 4 iterations of PubMedBERT that were obtained by training using different seeds. This results in an f1-challenge of 0.772 and f1-directions of 0.764. Additionally we observe that labels on which all 4 variations agree on had a much higher f1 averages across the variations compared to the 2-2 splits (0.867 and 0.864 vs. 0.37 and 0.304) which further indicates the value of solving disagreements on context relative to just reducing noise.             

Our suggested modelling, that is based on the systemic errors obtains better results over the finetuned baselines, however, the results of the oracle model shows there is much more room for future work that will be beneficial to our novel task and to figuring when classifiers should use the context in general.
